Combined Energy and Comfort Optimization of Air Conditioning System in Connected and Automated Vehicles

In this paper, we propose a combined energy and comfort optimization (CECO) strategy for the air conditioning (A/C) system of the connected and automated vehicles (CAVs). By leveraging the weather and traffic predictions enabled by the emerging CAV technologies, the proposed strategy is able to minimize the A/C system energy consumption while maintaining the occupant thermal comfort (OTC) within the comfort constraints, where the comfort is quantified by a modified predictive mean vote (PMV) model adapted for an automotive application. A general CECO problem is formulated and addressed using model predictive control (MPC) and weather/traffic previews. Depending on the ways of exploiting the preview information and enforcing the OTC constraint, different MPCs are developed based on solving different variations of the general CECO problem. The CECO-based MPCs are then tested in simulation using an automotive A/C system simulation model (CoolSim) as the virtual testbed. The simulation results show that, over SC03 driving cycle, the proposed CECO-based MPCs outperform the baseline cabin temperature tracking controller, reducing the A/C system energy consumption by up to 7.6%, while achieving better OTC according to the PMV-based metrics. This energy saving in A/C system translates to 3.1% vehicle fuel economy improvement. The trade-off between energy efficiency and OTC for different control scenarios is also highlighted.

==> asme2e <==


@article{art,
	author	=	"A. Author and
B. Author and C. Author",
	title	=	"Article {T}itle",
	journal =   "Journal
{N}ame",
	volume  =	1,
	number	=	5,
	pages   =   "1--3",
	month   =  
"May",
	year	=	1994}

@book{latex,
	author	  =	"L. Lamport",
	title	 
=	"\LaTeX: a Document Preparation System",
	publisher =
"Addison-Wesley",
	year	  =	1986,
	address   =	"Reading,
MA"}

@book{goosens,
	author	  =	"M. Goosens and F. Mittelbach and A.
Samarin",
	title	  =	"The \LaTeX\ Companion",
	publisher
=	"Addison-Wesley",
	address	  =	"Reading, MA",
	year	 
=	1994}

@booklet{blt,
	author	=	"A. Booklet",
	title	=	"Booklet
title",
	howpublished =   "On the WWW",
	address =	"at
\verb+http://www.abc.edu+",
	note	=	"PDF file",
	month   =  
"May",
	year	=	1994}

@inbook{ibk,
	editor    =	"A. Inbook",
	title	 
=	"Book title",
	chapter   = 1,
	pages     = "1--3",
	volume 
=	2,
	series	=	"{Series Title}",
	edition = "$1^{st}$",
	type    =
"{Chap.}",
	publisher =	"Publisher {N}ame",
	address   =	"Publisher
address",
	note      = "See also URL \verb+http://www.abc.edu+",
	year	 
=	1991}

@incollection{icn,
	author    =	"A. Incollection",
	title	 
=	"Article title",
	editor    =	"A. Editor",
	booktitle =	"Collection
{T}itle",
	chapter   = 1,
	pages     = "1--3",
	volume 
=	2,
	series	=	"Series title",
	month   =   "May",
	edition =
"$3^{rd}$",
	type    = "{C}hapter",
	publisher =	"Publisher
{N}ame",
	address   =	"Publisher address",
	note      = "See also URL
\verb+http://www.abc.edu+",
	year	  =	1991}

@inproceedings{ips,
	author   
=	"A. Inproceedings",
	title	  =	"Article title",
	editor    =	"A. Editor
and B. Editor",
	booktitle =	"Proceedings {T}itle",
	volume  =	"{\bf
1}",
	series	=	"Series name",
	pages     = "1--3",
	address   =	"Publisher
address",
	month   =   "May",
	organization =	"Organization
{N}ame",
	publisher =	"Publisher {N}ame",
	note      = "Paper number
1234",
	year	  =	1991}

@manual{asmemanual,
	author    =	"{ASME}",
	title	 
=	"{ASME} Manual {MS-4}, An {ASME} Paper",
	organization =	"The American
Society of Mechanical Engineers",
	edition  = "latest",
	address   =	"New
York",
	note      = "See also URL
\verb+http://www.asme.org/pubs/MS4.html+",
	year	 
=	2003}

@mastersthesis{mts,
     author = "A. Mastersthesis",
     title =
"{Thesis Title}",
     school = "University of Higher Education",
     year
= 2003,
     type = "{MS Thesis}",
     address = "Cambridge, {MA}",
    
month = "May",
     note = "See also URL
\verb+http://www.abc.edu+"}

@misc{mis,
     author = "A. Misc",
     title 
= "Miscellaneous {T}itle",
     howpublished = "On the WWW",
     month =
"May",
     year = "2003",
     note = "URL
\verb+http://www.abc.edu+"}

@phdthesis{pts,
     author = "A. Phdthesis",
 
   title = "{Thesis Title}",
     school = "University of Higher
Education",
     year = 2003,
     type = "{PhD Thesis}",
     address =
"Cambridge, {MA}",
     month = "May",
     note = "See also URL
\verb+http://www.abc.edu+"}

@proceedings{pro,
	title	  =	"Volume
{T}itle",
	year	  =	1991,
	editor    =	"A. Proceedings",
	volume   
=	1,
	series	  =	"Proceedings {S}eries",
	address   =	"Publisher
address",
	month   =   "May",
	organization =	"Organization
{N}ame",
	publisher =	"Publisher {N}ame",
	note      = "See also URL
\verb+http://www.abc.edu+"}

@techreport{trt,
     author = "A.
Techreport",
     title = "{Techreport title}",
     institution =
"University of Higher Education",
     year = "2003",
     type = "Progress
report",
     number = "1",
     address = "Cambridge, {MA}",
     month =
"May",
     note = "See also URL
\verb+http://www.abc.edu+"}

@unpublished{upd,
     author = "A.
Unpublished",
     title = "{Unpublished document title}",
     note = "See
also URL \verb+http://www.abc.edu+",
     month = "May",
     year = 2003}

